Analysis of Structured Deep Kernel Networks

In this paper, we leverage a recent deep kernel representer theorem to connect kernel based learning and (deep) neural networks in order to understand their interplay. In particular, we show that the use of special types of kernels yields models reminiscent of neural networks that are founded in the same theoretical framework of classical kernel methods, while benefiting from the computational advantages of deep neural networks. Especially the introduced Structured Deep Kernel Networks (SDKNs) can be viewed as neural networks (NNs) with optimizable activation functions obeying a representer theorem. This link allows us to analyze also NNs within the framework of kernel networks. We prove analytic properties of the SDKNs which show their universal approximation properties in three different asymptotic regimes of unbounded number of centers, width and depth. Especially in the case of unbounded depth, more accurate constructions can be achieved using fewer layers compared to corresponding constructions for ReLU neural networks. This is made possible by leveraging properties of kernel approximation.

==> chapters/app_numeric_details.tex <==
\section{Details of the numerical experiments} \label{sec:details_numerical_experiments}

\begin{table}[h]
\centering
%
\caption[Data sets.]{Overview of the model structures. Whenever available, setups from the literature were chosen for comparison reasons \tw{add references}. Otherwise, suitable setups are used.} 
\renewcommand{\arraystretch}{1.4}
\tiny
\begin{tabular}{|l|r|r|l|l|} \hline
Data set & setup & \# para NN & \# para SDKN\\ \hline \hline
cpusmall & [12, 32, 16, 1] & ? & ? \\
cycle power plant & [4, 32, 32, 16, 1] & ? & ?  \\ 
cadata & [8, 32, 16, 1] & ? & ?  \\ \hline
Letter Recognition & [15, 32, 32, 32, 26] & ? & ? \\
MNIST & [784, 500, 150, 10] & ? & ? \\
Covtype & [54, 128, 128, 32, 7] & ? & ?   \\
SUSY & [18, 300, 300, 300, 300, 2]  & ? & ? \\
Higgs & [28, 300, 300, 300, 300, 2]  & ? & ? \\ \hline
\end{tabular}
\label{tab:numerical_results_mnist}
\end{table}


\begin{table}[h]
\centering
%
\caption[Benchmark of SDKN vs NN - Overview optimization times.]{Benchmark of SDKN vs NN on several data sets: Depicted is the training time per epoch.} 
\renewcommand{\arraystretch}{1.4}
\tiny
\begin{tabular}{|l|l|l|l|l|l|l|} \hline
 & data set & ReLU NN & ELU NN & Gaussian & Matern & Wendland \\ \hline \hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{MSE}} & cpusmall & $0.038 \pm 0.0113$s & $0.033 \pm 0.0120$s & $0.224 \pm 0.0597$s & $0.223 \pm 0.0388$s & $0.179 \pm 0.0282$s  \\
& Cycle power plant & $0.040 \pm 0.0148$s & $0.046 \pm 0.0132$s & $0.348 \pm 0.0879$s & $0.364 \pm 0.0372$s & $0.199 \pm 0.0234$s   \\
& Cadata & $0.043 \pm 0.0053$s & $0.049 \pm 0.0049$s & $0.426 \pm 0.1127$s & $0.471 \pm 0.0732$s & $0.267 \pm 0.1027$s  \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{Error}} & letter recognition & $0.084 \pm 0.0146$s & $0.228 \pm 0.0327$s & $0.940 \pm 0.0974$s & $0.970 \pm 0.1040$s & $0.806 \pm 0.0938$s \\
& MNIST & $1.859 \pm 0.2150$s & $1.583 \pm 0.0624$s & $2.349 \pm 0.0960$s & $2.230 \pm 0.1123$s & $2.169 \pm 0.0981$s \\
& Covertype & $2.870 \pm 0.0556$s & $8.385 \pm 0.3285$s & $11.263 \pm 0.2299$s & $10.518 \pm 0.1883$s & $10.548 \pm 0.3455$s   \\
& SUSY & Not yet computed & as this will take & quite some time & (huge dataset). & Want to wait \\
& HIGGS & for your feedback & first whether & experiments are & reasonable. &  \\
 \hline \hline
\end{tabular} \label{tab:numerical_results_time}
\end{table}


\begin{table}[h]
\centering
%
\caption[Benchmark of SDKN vs NN - Overview trained epochs.]{Benchmark of SDKN vs NN on several data sets: Depicted is the number of epochs until the stop.} 
\renewcommand{\arraystretch}{1.4}
\tiny
\begin{tabular}{|l|l|l|l|l|l|l|} \hline
 & data set & ReLU NN & ELU NN & Gaussian & Matern & Wendland \\ \hline \hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{MSE}} & cpusmall & $76.3 \pm 15.4$ & $125.0 \pm 25.9$ & $102.7 \pm 17.4$ & $116.5 \pm 13.7$ & $92.2 \pm 18.8$  \\
& Cycle power plant & $41.0 \pm 11.0$ & $38.2 \pm 4.6$ & $49.2 \pm 15.2$ & $63.4 \pm 12.8$ & $49.0 \pm 10.6$ \\
& Cadata & $81.1 +- 20.4$ & $73.6 +- 12.3$ & $80.5 +- 14.0$ & $73.7 +- 12.5$ & $71.4 +- 9.0$ \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{Error}} & letter recognition & $153.0 \pm 15.2$ & $145.4 \pm 18.9$ & $86.3 \pm 7.6$ & $87.2 \pm 9.0$ & $76.7 \pm 9.6$\\
& MNIST & $23.9 \pm 3.0$ & $20.2 \pm 1.4$ & $15.5 \pm 1.9$ & $16.6 \pm 2.1$ & $16.7 \pm 2.1$ \\
& Covertype & $92.7 \pm 9.9$ & $90.3 \pm 15.0$ & $69.6 \pm 6.9$ & $75.4 \pm 12.3$ & $71.2 \pm 10.0$   \\
& SUSY & Not yet computed & as this will take & quite some time & (huge dataset). & Want to wait \\
& HIGGS & for your feedback & first whether & experiments are & reasonable. &  \\
 \hline \hline
\end{tabular} \label{tab:numerical_results_epochs}
\end{table}

\textcolor{blue}{Maybe show a table with the total optimization time instead of the time per epoch?} \todo{do this}




==> chapters/numerical_investigation.tex <==
\section{Numerical investigations} \label{sec:numerical_exp}

The first section provides some information about the available implementation of the SDKN. Section \ref{subsec:visualization_activ_func} illustrates the interpretation of the single-dimensional kernel mappings as optimizable activation functions. Finally, Section \ref{subsec:benchmark_comparison} provides a thorough comparison of the proposed SDKNs with standard Neural Networks on a range of standard machine learning data sets.

\subsection{Implementation details} \label{subsec:implementation_details}

An implementation of the SDKN model can be found at \cite{codeSDKN}, which is built using the open-source machine learning framework Pytorch \cite{NEURIPS2019_9015}. The most important part is the implementation of the activation function layers, which can be realized with standard operations. We remark that these layers can be used as any other PyTorch module and can thus be combined with existing methods. Especially the code is compatible with other modules like data management tools and optimizers of PyTorch or other standard machine learning techniques. For example DropOut can be used for regularization. As this is only applied during training, it does not harm the mathematical foundation based on the Deep Kernel representer theorem.

\subsection{Visualization of optimizable activation function} \label{subsec:visualization_activ_func}

As motivated in Section \ref{subsubsec:overall_setup}, the single-dimensional kernel layers give rise to an interpretation via optimizable activation functions. To illustrate this, several of such mappings are depicted in Figure \ref{fig:visualization_activ_funcs} for the Gaussian and the Wendland $k=0$ kernel after training on the so called letter recognition data set. For this, the settings as described in the next Section \ref{subsec:benchmark_comparison} were applied, especially $M=3$ centers were used. These centers are visualized as crosses in Figure \ref{fig:visualization_activ_funcs}. The kernel mappings within the first dimension of the first, second and third single-dimensional layer are depicted from left to right. 

Both the initial shape (dashed, red line) as well as the final shape (solid, green) of the optimizable activation functions are provided to visualize the changes during training. The background bar plot visualizes the distribution of the training samples. The Figures are similar to that in \cite{SCARDAPANE201919} and thus allow for a comparison. As the centers are a subset of the training samples, the single-dimensional kernel function has a meaningful shape in the domain where the data points are distributed. \todo{At some point discuss the non monotonicity of the functions}

It \todo{Improve plots, same ranges!} can be seen that initially (red) the training samples are distributed only on a smaller range, especially in later layers\todo{This could be related to a bad initialization of the activation function parameters?}. This is in contrast to the distribution of the training samples after the optimization, which are on a wider range. Furthermore, the optimized activation functions look way more reasonable. The different shapes and smoothness for the Gaussian (top) and the Wendland kernel (bottom) can be easily recognized. The use of more center points, e.g.\ $M > 3$ yields to more involved activation functions. However this was not found to be significantly superior in numerical experiments. 

We remark that the single-dimensional kernel layers can be initialized such that they approximate some known activation function in the beginning. Due to the approxmation properties of kernel methods this works especially well when using multiple centers.

\begin{figure}
\begin{center}
\includegraphics[width=0.32\textwidth]{Figures/png_activ_funcs/visualization_activ_func_gaussian_1.png}
\includegraphics[width=0.32\textwidth]{Figures/png_activ_funcs/visualization_activ_func_gaussian_2.png}
\includegraphics[width=0.32\textwidth]{Figures/png_activ_funcs/visualization_activ_func_gaussian_3.png}
\includegraphics[width=0.32\textwidth]{Figures/png_activ_funcs/visualization_activ_func_wendland_1.png}
\includegraphics[width=0.32\textwidth]{Figures/png_activ_funcs/visualization_activ_func_wendland_2.png}\includegraphics[width=0.32\textwidth]{Figures/png_activ_funcs/visualization_activ_func_wendland_3.png}
\end{center}
\caption{Visualization of several single-dimensional kernel activation function before (red) and after (green) optimization. The columns refer to one dimension within the first, second respective third single-dimensional kernel function  layer. Top: Gaussian kernel, bottom: Wendland $k=0$ kernel. The histograms visualize the distribution of the training data after the optimization.}
\label{fig:visualization_activ_funcs}
\end{figure}




\subsection{Benchmark comparison} \label{subsec:benchmark_comparison}

In this section a benchmark comparison of the NN and the SDKN approach in various regression, binary as well as multiclass classification tasks is presented.

\subsubsection{Experimental setup}
%
The investigated data sets are summarized in Table \ref{tab:numerical_results_mnist}, consisting of standard machine learning data sets. Though the MNIST data set is a set of images, no convolutional layers were applied, i.e.\ a permutation invariant representation approach was employed. \\
%
In order to have a fair and simple comparison, both the NNs and the SDKNs use the same network architecture: For the NNs, Instead of the
single-dimensional kernel function layers, simply an activation function is applied.  If available in the literature, the same or similar setups have been chosen, such that a comparison is possible. The SDKN uses $M=3$ centers within the single-dimensional kernel layers, which are randomly chosen from the training set. An overview of the used models including depth and widths is given in the Appendix \ref{sec:details_numerical_experiments}. \\
%
The initialization of the optimizable parameters was done via the He-initialization. Regarding the optimization, batch learning with a batch size of 256 and a maximal number of epochs of 200 was used. The Adam optimizer was chosen with an initial learning rate of $10^{-3}$ (default value). A learning rate scheduler halves the learning rate if the validation loss does not improve for $2$ epochs. For regularizaton we employed early stopping using a patience of $5$ epochs concerning a relative improvement of at least $10^{-3}$ on the validation loss. No model-specific hyperparameter tuning or various advanced deep learning training methods were applied. The computations were run on a machine with Intel i7-9700K CPU 8 core and 32GB memory.


\begin{table}[h]
\centering
%
\caption[Data sets.]{Considered data sets. If no test data was provided, 20\% of the whole data set were randomly chosen for testing. 15\% of the training data were used as validation set to determine the early stopping. The input dimensionality is given in the column \textit{Dimension} and the task of the data set is given in the penultimate column (Reg = Regression, MC-7 = Multi Class Classification with 7 classes, BC = Binary Classification)} 
\renewcommand{\arraystretch}{1.4}
\tiny
\begin{tabular}{|l|r|r|l|l|l|} \hline
Data set & Data size & Test size & Dimension & Type & Source \\ \hline \hline
Cpusmall & $8192$ & 20\% & 12 & Reg & LIBSVM  \\
Cycle Power Plant & 9568 & 20\% & 4 & Reg & UCI \\ 
Cadata & $20640$ & 20\% & 8 & Reg & LIBSVM  \\ \hline
Letter Recognition & $1.6 \cdot 10^4$ & $4 \cdot 10^3$ & 15 & MC-26 & UCI \\
MNIST & $7 \cdot 10^4$ & $10^4$ & 724 & MC-10 & MNIST \\
Covertype & $5.81 \cdot 10^5$ & 20\% & 54 & MC-7 & UCI \\
SUSY & $5 \cdot 10^6$  & $5 \cdot 10^5$ & 18 & BC & UCI  \\
HIGGS & $1.1 \cdot 10^7$ & $5 \cdot 10^5$ & 28 & BC & UCI \\ \hline
\end{tabular}
\label{tab:benchmark_datasets}
\end{table}


\subsubsection{Results}

The results of the comparison of NN and SDKN on the benchmark data sets are summarized in Table \ref{tab:numerical_results_benchmark}. For each data set the optimization of each model was done 10 times to lower the randomness due to the initial initialization of the parameters. The evaluation of the models was done on test sets that are distinct from the training sets. The table states the mean value plusminus the standard deviation of the final optimized models.

From the results within the table it is evident that the SDKN reaches accuracy on par or superior to the Neural Networks for the considered data sets. We want to remark that the training time per epoch of the SDKN is larger than for the NN. This is clearly related to the additional operations required in the computation of the single-dimensional kernel function layers. The additional training time is in the range of a factor of $2-10$, depending on various quantities like the network size. On the other hand, the computation of the SDKN often terminates earlier for larger datasets. Thus, the ratio of the total optimization time is not that large when dealing with large data sets. Precise numbers are given in the Appendix \ref{sec:details_numerical_experiments}, cf.\ Tables \ref{tab:numerical_results_time} and \ref{tab:numerical_results_epochs}.

\textcolor{blue}{
\begin{enumerate}
\item Is a statement on the evaluation time interesting?
\item Time measurement might not be completly accurate, since computer was partly used in parallel (for computationaly inexpensive tasks like mails and writing)
\end{enumerate}
}

Finally we remark that it will be for sure possible to adjust and optimize the setup of either the NN or the SDKN to achieve superior results compared to the other approach. This is possible due to the huge range of hyperparameters like the way of weight initialization, widths and depth of the network, choice of activation function respective kernel, optimizer, learning rate, regularization and so on. \\
However as the results were achieved without any model specific setup optimization, we consider them to provide a fair assessment of their learning qualities. \todo{Compare with literature accuracy}

%
%
%
%
%

\begin{table}[h]
\centering
%
\caption[Benchmark of SDKN vs NN.]{Benchmark of SDKN vs NN on several data sets. Depicted is the test loss (MSE) or the test error (Error) over 10 runs.} 
\renewcommand{\arraystretch}{1.4}
\tiny
\begin{tabular}{|l|l|l|l|l|l|l|} \hline
 & data set & ReLU NN & ELU NN & Gaussian & Matern & Wendland \\ \hline \hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{MSE}} & cpusmall & $(4.12 \pm 0.1) 10^{-3}$ & $(4.46 \pm 0.09) 10^{-3}$ & $(3.92 \pm 0.15) 10^{-3}$ & $(3.78 \pm 0.15) 10^{-3}$ & $(3.74 \pm 0.18) 10^{-3}$ \\
& Cycle power plant & $(1.31 \pm 0.1) 10^{-2}$ & $(1.37 \pm 0.01) 10^{-2}$ & $(1.32 \pm 0.02) 10^{-2}$ & $(1.26 \pm .03) 10^{-2}$ & $(1.28 \pm 0.02) 10^{-2}$ \\
& Cadata & $(6.25 \pm 0.12 ) 10^{-2}$ & $(6.90 \pm 0.05) 10^{-2}$ & $(5.49 \pm 0.12) 10^{-2}$ & $(5.22 \pm 0.12) 10^{-2}$ & $(5.29 \pm 0.09) 10^{-2}$ \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{Error}} & letter recognition & $12.21 \pm 0.86 \%$ & $10.22 \pm 0.58 \%$ & $8.17 \pm 0.47 \%$ & $10.36 \pm 0.75\%$ & $8.65 \pm 0.46\%$ \\
& MNIST & $1.89 \pm 0.08\%$ & $1.86 \pm 0.07\%$ &  $2.11 \pm 0.18\%$ & $1.93 \pm 0.12\%$ & $2.11 \pm 0.15\%$ \\
& Covertype & $10.11 \pm 0.49\%$ & $8.27 \pm 0.48\%$ &  $4.63 \pm 0.28\%$ & $4.99 \pm 0.20\%$ & $4.60 \pm 0.18\%$ \\
& SUSY & Not yet computed & as this will take & quite some time & (huge dataset). & Want to wait \\
& HIGGS & for your feedback & first whether & experiments are & reasonable. &  \\
 \hline \hline
\end{tabular} \label{tab:numerical_results_benchmark}
\end{table}



\newpage


